Generating Adversarial Point Clouds Using Diffusion Model

Adversarial attack methods for 3D point cloud classification reveal the vulnerabilities of point cloud recognition models. This vulnerability could lead to safety risks in critical applications that use deep learning models, such as autonomous vehicles. To uncover the deficiencies of these models, researchers can evaluate their security through adversarial attacks. However, most existing adversarial attack methods are based on white-box attacks. While these methods achieve high attack success rates and imperceptibility, their applicability in real-world scenarios is limited. Black-box attacks, which are more meaningful in real-world scenarios, often yield poor results. This paper proposes a novel black-box adversarial example generation method that utilizes a diffusion model to improve the attack success rate and imperceptibility in the black-box setting, without relying on the internal information of the point cloud classification model to generate adversarial samples. We use a 3D diffusion model to use the compressed features of the point cloud as prior knowledge to guide the reverse diffusion process to add adversarial points to clean examples. Subsequently, its reverse process is employed to transform the distribution of other categories into adversarial points, which are then added to the point cloud.

==> Body/0Abstract.tex <==
Adversarial attack methods for 3D point cloud classification reveal the vulnerabilities of point cloud recognition models. This vulnerability could lead to safety risks in critical applications that use deep learning models, such as autonomous vehicles. To uncover the deficiencies of these models, researchers can evaluate their security through adversarial attacks. However, most existing adversarial attack methods are based on white-box attacks. While these methods achieve high attack success rates and imperceptibility, their applicability in real-world scenarios is limited. Black-box attacks, which are more meaningful in real-world scenarios, often yield poor results. This paper proposes a novel black-box adversarial example generation method that utilizes a diffusion model to improve the attack success rate and imperceptibility in the black-box setting, without relying on the internal information of the point cloud classification model to generate adversarial samples. We use a 3D diffusion model to use the compressed features of the point cloud as prior knowledge to guide the reverse diffusion process to add adversarial points to clean examples. Subsequently, its reverse process is employed to transform the distribution of other categories into adversarial points, which are then added to the point cloud.
Furthermore, density-aware Chamfer distance is incorporated to constrain the noise added during back-propagation, further improving the imperceptibility of adversarial examples. Experimental results demonstrate that the proposed method exhibits high attack performance against various point cloud recognition models and defense methods, significantly enhancing the effectiveness of black-box attacks. In the black-box scenario, the attack success rate can reach about 90\%. The code for this work is available at: \url{https://github.com/AdvPC/Generating-Adversarial-Point-Clouds-Using-Diffusion-Model}.

% \jz{here you need to highlight the statistics of how much improved in terms of attack effectiveness compared with SOTA otherwise significant seems not supported}.


==> Body/5_Exper.tex <==

In this section, we present the experiment settings, experimental results, and ablation studies. Before elaborating on experimental details, we first set up research questions.

\subsection{Research Questions}
In this work, we explored generating point cloud AEs with diffusion models. To examine the attack success rate, concealment, and transferability of our method. We evaluate the method with the following research questions (RQs).
\begin{itemize}
    \item \textit{RQ1:} \textcolor{blue}{Given the limited research on generating 3D adversarial examples, can we use diffusion models to generate effective adversarial examples across different datasets and models, Such as PointNet++ and the ModelNet40 dataset?}
    \item \textit{RQ2:} \textcolor{blue}{Explore whether different diffusion steps and noise constraints affect the performance of generated adversarial examples?}

    \item \textit{RQ3:} \textcolor{blue}{Can the 3D diffusion scheme generate adversarial examples resistant to defense when faced with different models?}

\end{itemize}


\begin{figure}[!t]
    \centering
    \includegraphics[width=0.5\textwidth]{image/ASR_1.pdf}
    \caption{The impact of noise EPS on Chamfer Distance and attack success rate}
    \label{fig:asr}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=3in]{image/attack_success_rate.pdf}
\caption{Fix the amount of noise added by diffusion at each step and optimize the effect of the number of times on the performance of the attack, which targets the network as PointNet++.}
\label{fig:experiment_OP_ASR}
\end{figure}




\begin{table*}[t]
\footnotesize
\centering
\caption{ASR (\%) of different attack methods with and without defense on  ModelNet40 (MN).}
    \begin{tabular}
    {lcp{10mm}<{\centering}p{10mm}<{\centering}p{10mm}<{\centering}p{10mm}<{\centering}p{10mm}<{\centering}p{10mm}<{\centering}p{10mm}<{\centering}p{10mm}<{\centering}p{10mm}<{\centering}p{10mm}<{\centering}p{10mm}<{\centering}p{10mm}<{\centering}p{10mm}<{\centering}}
        \toprule
        \multirow{3}{*}{Proxy Model}
        & \multirow{3}{*}{data}
        & \multirow{3}{*}{Defense}
        & \multicolumn{8}{c}{Attack Method} 
        \\
        \cmidrule(lr){4-12}
        & &  & \makecell{Drop\\-400} & \makecell{CW\\($l_2$)} & \makecell{CW\\(CD)} &\makecell{CW\\(HD)}& GeoA3 & AdvPC& \makecell{LG\\-GAN} & DPMA & Ours
        \\
        \midrule
        \multirow{3}{*}{PointNet} & \multirow{3}{*}{MN} & - & 59.64  & \textbf{100.00}  &  \textbf{100.00} & \textbf{100.00}  & \textbf{100.00}  & \textbf{100.00}  & 99.22  & 93.80  &  94.20
        \\
        &   & SRS & 58.14 & 53.00  & 67.19  & 69.94  & 81.65  & \textbf{98.87}  & 92.13  & 93.48 & 90.43    
        \\
         &   & SOR & 56.28 & 13.82  & 15.63   & 15.80  & 42.79  & 46.19  & 67.25 & 87.00  &   \textbf{93.06}
        \\
        \midrule
        \multirow{3}{*}{Dgcnn} & \multirow{3}{*}{MN} & - &  45.91 & \textbf{100.00}  & \textbf{100.00}  &  \textbf{100.00}   & \textbf{100.00} & 94.58  &  86.08 &97.45 & 95.23 
        \\
        &  & SRS &35.05   & 31.09  &  37.11 & 32.29  & 77.71  & 70.63  & 80.60  & \textbf{94.73}  & 92.40  
        \\
        &  & SOR &15.03   & 2.26  & 2.92  & 3.13  & 56.25  & 11.04  & 50.17  & 93.11  & \textbf{94.60}
        \\
        \midrule
        \multirow{3}{*}{PointConv} & \multirow{3}{*}{MN} & - & 37.12 &\textbf{100.00}  &  \textbf{100.00} & \textbf{100.00}  & 96.09 & 98.54  &  78.04 & 94.98   & 94.50
        \\
        &  & SRS  & 35.09  & 37.29  & 28.95  &  27.77 & 21.48  & 93.54  &  71.88 & \textbf{94.06} & 92.60
        \\
        & & SOR  & 34.44 & 18.13  & 17.29  & 19.16 &18.35  & 91.25 & 63.88  & 90.71  & \textbf{93.21}
        \\
        \bottomrule
    \end{tabular}
    % }
    % \vspace{0.5em}
    
    \label{tab:wh}
    % \vspace{-0.5em}
\end{table*}


\begin{table*}[!t]
\centering
\renewcommand{\tablename}{Fig}
\begin{tabular}{c c c c c }
\textbf{Clean}& \textbf{FGSM}& \textbf{IFGSM} & \textbf{SI-query} & \textbf{Ours} \\
% \vspace{0.01mm}
\adjustbox{valign=c}{\includegraphics[width=2.3cm]{image/result/bench-clean.png}}
&  \adjustbox{valign=c}{\includegraphics[width=2.3cm]{image/result/bench-fgsm.png}}
& \adjustbox{valign=c}{\includegraphics[width=2.3cm]{image/result/bench-ifgsm.png}}
&  \adjustbox{valign=c}{\includegraphics[width=2.3cm]{image/result/bench-siquery.png}}
& \adjustbox{valign=c}{\includegraphics[width=2.3cm]{image/result/bench-ours-airplane.png}} \vspace{-0.4cm} \\ \vspace{0.5cm}
bench & table & bench & chair & airplane \\ 
\adjustbox{valign=c}{\includegraphics[width=2.1cm]{image/result/desk-clean.png}} 
&\adjustbox{valign=c}{\includegraphics[width=2.1cm]{image/result/fgsm-desk-curtain.png}}      
&  \adjustbox{valign=c}{\includegraphics[width=2.1cm]{image/result/ifgm-desk-sink.png}}
&  \adjustbox{valign=c}{\includegraphics[width=2.5cm]{image/result/siquery-radio.png}}
& \adjustbox{valign=c}{\includegraphics[width=2.0cm]{image/result/ours-bed.png}} \vspace{0cm} \\ \vspace{0.5cm}
desk & curtain & sink & radio & bed \\
\adjustbox{valign=c}{\includegraphics[width=2.1cm]{image/result/vase.png}}   
& \adjustbox{valign=c}{\includegraphics[width=2.1cm]{image/result/vase-fgsm-flower-pot.png}}
& \adjustbox{valign=c}{\includegraphics[width=2.0cm]{image/result/vase-ifgm.png}}
& \adjustbox{valign=c}{\includegraphics[width=2.1cm]{image/result/vase-ours-xbox.png}}
& \adjustbox{valign=c}{\includegraphics[width=2.0cm]{image/result/ours-flow-pot.png}}\vspace{0cm} \\ \vspace{0.3cm}
vase & vase & flower-pot & Xbox & flower-pot \\
\adjustbox{valign=c}{\includegraphics[width=2.0cm]{image/result/bottle.png}} 
& \adjustbox{valign=c}{\includegraphics[width=2.0cm]{image/result/fgsm-bottle-xbox.png}} 
&\adjustbox{valign=c}{\includegraphics[width=2.1cm]{image/result/bottle-vase-ours.png}} 
& \adjustbox{valign=c}{\includegraphics[width=2.0cm]{image/result/bottle-vase.png}} 
& \adjustbox{valign=c}{\includegraphics[width=2.0cm]{image/result/bottle-vase-our.png}}  \vspace{0cm} \\ \vspace{0.3cm}
bottle & Xbox & vase & vase & vase \\
\adjustbox{valign=c}{\includegraphics[width=2.0cm]{image/result/bowl.png}}
&\adjustbox{valign=c}{\includegraphics[width=2.0cm]{image/result/fgsm-plant.png}}
&\adjustbox{valign=c}{\includegraphics[width=2.0cm]{image/result/bowl--chair-ifgm.png}}
&\adjustbox{valign=c}{\includegraphics[width=2.0cm]{image/result/SI-query-plant.png}}
& \adjustbox{valign=c}{\includegraphics[width=2.0cm]{image/result/table-ours.png}} \vspace{-0.4cm} \\ \vspace{0.5cm}
bowl & plant & chair & plant &table 
\end{tabular}
\caption{Comparison of various attack methods.}
\label{tab:exp_result}
\end{table*}


\subsection{Experimental Settings }
\textbf{Datasets. }
For a fair comparison, we evaluate AEs generated by our method on ShapeNet and ModelNet40 as prior works \cite{huang2022shape}. We assess the attack performance on ShapeNet, which includes approximately 50,000 3D CAD models across 14 major and 55 subcategories, with each model containing at least 2,000 points \cite{chang2015shapenet}. Additionally, we evaluate our approach on ModelNet40, consisting of 12,311 CAD models from 40 object categories, with 9,843 for training and 2,468 for testing \cite{sun2022modelnet40}. Each object in ModelNet40 is uniformly sampled to 2,048 points and rescaled to a unit cube. Data augmentation techniques, such as random scaling and jittering, are applied to preprocess the point clouds in the test set.

 \textit{RQ2: }We report the attack access rate with non-defense on ModelNet40 and ShapeNet. While ModelNet40 shows more distinguishable results than ShapeNet, we report the results of the rest tasks on ModelNet40. For ModelNet40, we chose three surrogate models for black-box transfer-based attack evaluation and compared them with our proposed approach. For ShapeNet, we use the proposed method to evaluate the attack performance of two models.

 \noindent \textbf{Models. } 
Our approach is evaluated on six benchmark 3D recognition models: PointNet \cite{qi2017pointnet}, PointNet++(MSG) \cite{qi2017pointnet++}, PointConv \cite{wu2019pointconv}, Pct \cite{guo2021pct}, DGCNN \cite{wang2021object}, and Curvenet \cite{muzahid2020curvenet}. These models were chosen for their unique architectures and established performance in 3D recognition tasks. 

\textbf{1, }PointNet uses a symmetric function for permutation invariance, while PointNet++ introduces hierarchical feature learning. 

\textbf{2, }PointConv enhances feature representation with a point cloud-specific convolution, and Pct excels with a transformer-based architecture. 

\textbf{3, }DGCNN captures local structures with dynamic graph construction. 

\textbf{4, }Curvenet uses 3D curves for feature extraction. 

We selected PointNet, DGCNN, and Pct as proxy models to conduct comparative tests on PointNet++, Curvenet, and PointConv, evaluating our approach's robustness with and without defense measures. This evaluation across diverse architectures allows us to assess the generalizability and effectiveness of our method, providing insights into its performance against various 3D recognition systems.

\noindent \textbf{Attack Method. }

We leverage a pre-trained open-source 3D-diffusion model, trained on extensive point cloud data, as the basis for our manifold attack and compare our approach (Ours) with eight baseline methods.  These include the deletion-based method Drop-400 \cite{zheng2019pointcloud}, which drops the most critical 400 points, and perturbation-based methods using optimization like C$\&$W under \( l_2 \)-norm, Chamfer distance (CD), and Hausdorff distance (HD) constraints \cite{xiang2019generating}. Additionally, we consider GeoA3 \cite{wen2020geometry}, which applies geometric-aware constraints, and AdvPC \cite{hamdi2020advpc}, which focuses on high transferability. We also compare against generative-based methods such as LG-GAN \cite{zhou2020lg} and DPMA \cite{tang2023deep}.
For attack performance testing, we select the best configuration of these adversarial attack methods to achieve the best attack success rate\cite{tang2023deep} they can achieve. Due to time constraints, we selected only FGSM, IFGSM, and PGD as comparative experiments for evaluating stealthiness.

\noindent \textbf{Evaluation Metrics. }
We begin by statistically analyzing the attack success rate (ASR) of the generated adversarial samples on the 3D point cloud recognition model to evaluate the method's effectiveness. To assess the imperceptibility and efficacy of the generated adversarial point clouds, we compute the Hausdorff Distance and Chamfer Distance between the original point cloud and the adversarial output. The Hausdorff Distance quantifies the maximum deviation between point sets, while the Chamfer Distance measures the average displacement, providing insights into the subtlety of the perturbations. The formula is defined as follows.
\begin{equation}
    \text{ASR} = \frac{\sum_{i=1}^{N} \mathbb{I}(Y_i \neq \hat{Y}_i)}{N} \times 100\% ,
\label{ASR}
\end{equation}
\begin{equation}
    \mathcal{D}_{C}\left(X, X^{\prime}\right)=\frac{1}{\left\|X^{\prime}\right\|_{0}} \sum_{y \in X^{\prime}} \min _{x \in X}\|x-y\|_{2}^{2}
    \label{CD}
\end{equation}
\begin{equation}
    \mathcal{D}_{H}\left(X, X^{\prime}\right)=\max _{y \in X^{\prime}} \min _{x \in X}\|x-y\|_{2}^{2},
    \label{HD}
\end{equation}
In these formulas, \(X\) represents the original point cloud, and \(X'\) denotes the adversarial point cloud. Equation \ref{ASR} defines the Attack Success Rate (ASR), which quantifies the percentage of perturbed samples misclassified by the model. \(Y_i\) and \(\hat{Y}_i\) represent the true and predicted labels, respectively, and \(N\) is the total number of samples. Equation \ref{CD} defines the Chamfer Distance (\(\mathcal{D}_C\)), which calculates the average displacement between points in \(X\) and \(X'\). Equation \ref{HD} defines the Hausdorff Distance (\(\mathcal{D}_H\)), which measures the maximum deviation between points in the two sets. The ASR, defined in Equation \ref{ASR}, quantifies the ratio of perturbed examples incorrectly classified by the black-box transfer-based attacked model. Evaluating our attack in terms of effectiveness, stealthiness, and transferability offers a comprehensive understanding of its impact on 3D recognition models.


\begin{itemize}
    \item \emph{Effectiveness}: Measured by the attack success rate (ASR), which reflects the percentage of adversarial examples that successfully mislead the target model. A higher ASR indicates a more effective attack.
    \item \emph{Stealthiness}: Assessed using the Hausdorff distance and Chamfer distance to ensure that the generated adversarial examples are imperceptible and maintain a high degree of similarity to the original point clouds.
    \item \emph{Transferability}: Evaluated by testing the adversarial examples on different models to determine the robustness and generalization of the attack across various 3D recognition systems.
\end{itemize}

\textit{RQ1: }In order to test whether our proposed method can generate effective adversarial point clouds on different datasets, we tested it on both ModelNet40 and ShapeNet datasets. The test results of ModelNet40 can be found in Tab \ref{tab:wh}, and the test results of ShapeNet dataset are shown in Tab \ref{tab:table4}.
\textit{RQ3: }We use ablation experiments to find out the impact of different diffusion steps and noise constraints on the attack performance of generated adversarial examples. Details can be seen in Ablation Studies

\subsection{Experimental Results}
\jz{current we have shown some key statistics which are good, but more importantly I would like to see some typical and concrete adversarial examples where we are better than the SOTA attacks. Similarly, when discussing the defense approaches, I would like to see concrete adversarial examples which skip the defense detections.  Also, some limitations need to be discussed which can solicit insights and future directions}
\textbf{Performance Comparison with White Box Attacks and Generative Attacks. }
 The result in Tab \ref{tab:wh} shows that Drop-400 performs the worst. Among them, the three CW attacks (using l2, Chamfer Distance, and Hausdorff Distance as loss functions), GeoA3, and AdvPC all showed a 100\% success rate on PointNet. In particular,  LG-GAN \cite{zhou2020lg}, DPMA \cite{tang2023deep} and our method also successfully attacked these models, but the success rate was slightly lower than the previous methods. This is because the previous methods are white-box attack methods, which can use the gradient information of the attacked model, which greatly improves the success rate of the attack. However, our proposed method differs from LGAN and DPMA in that our method does not use any information from the attacked model, and our method is dataset-oriented rather than sample-oriented. In addition, the attack success rate of AdvPC on Dgcnn and PointConv did not reach 100\%, due to the trade-off imposed by auto-encoder for transferability.

\textbf{Black-box Performance And Comparison. } 
We comprehensively compare our 3D diffusion black-box attack with various baselines, including regular optimization-based attacks such as FGSM, IFGSM, and PGD. Specifically, our method is implemented with a reverse diffusion step size of 100 and $1t$ DCD optimization iterations, while all baselines adopt untargeted attacks with $\epsilon$ set to 0.32. The comparisons are conducted on the same RTX 3050 GPU, evaluating metrics such as attack success rate (ASR), Chamfer distance (CD), and Hausdorff distance (HD). The results listed in Table \ref{tab:table1} show that our method incurs the least geometric distance cost to achieve nearly 90\% ASR, with a lower time budget compared to regular optimization-based attacks. This aligns with our intuition that the diffusion model better preserves the point features from the original point clouds during adversarial example generation.

To evaluate the generalizability of these attack methods, we assessed the performance of adversarial point clouds after careful data preprocessing and measured the attack's success rate (ASR) across different models. The results demonstrate that our proposed diffusion attack consistently outperforms other methods in most cases in terms of ASR, CD, and HD, indicating its robustness and effectiveness across various 3D recognition models.
\begin{table*}[!htb]
    % \setlength{\belowcaptionskip}{1cm}
    % \scriptsizes
	\footnotesize
    \centering
        \caption{Quantitative comparison between our diff attack and existing black-box transfer-based attacks in terms of attack success rate (ASR), Chamfer distance (CD), Hausdorff distance (HD), and the proxy model used, where CD is multiplied by $10^2$ and HD is multiplied by $10^2$ for better comparison.}
    \setlength{\tabcolsep}{1mm}{
    \begin{tabular}{lcp{10mm}<{\centering}p{10mm}<{\centering}p{10mm}<{\centering}p{10mm}<{\centering}p{10mm}<{\centering}p{10mm}<{\centering}p{10mm}<{\centering}p{10mm}<{\centering}p{10mm}<{\centering}p{10mm}<{\centering}p{10mm}<{\centering}p{10mm}<{\centering}p{10mm}<{\centering}}
        \toprule
        \multirow{3}{*}{Proxy Model}
        & \multirow{3}{*}{Attack}
        & \multirow{3}{*}{Defense}
        & \multicolumn{3}{c}{PointNet++ \cite{qi2017pointnet++}} 
        & \multicolumn{3}{c}{Curvenet \cite{muzahid2020curvenet}}
        & \multicolumn{3}{c}{PointConv \cite{wu2019pointconv}}
        \\
        \cmidrule(lr){4-6}\cmidrule(lr){7-9}\cmidrule(lr){10-12}
        & & & ASR$\uparrow$ & CD$\downarrow$ & HD$\downarrow$ & ASR$\uparrow$ & CD$\downarrow$ & HD$\downarrow$ & ASR$\uparrow$ & CD$\downarrow$ & HD$\downarrow$  
        \\
        & & & (\%) & ($10^{-2}$) & ($10^{-2}$) & (\%) & ($10^{-2}$) & ($10^{-2}$) & (\%) & ($10^{-2}$) & ($10^{-2}$) 
        \\
        \midrule
        \multirow{3}{*}{PointNet \cite{qi2017pointnet}} & FGSM \cite{sen2023adversarial}  & - & 68.2 & 2.93 & 12.3 &  75.7 & \textbf{0.60}  & \textbf{5.04}  & 71.9  & 2.18  & 17.06  
        \\
        & IFGSM \cite{you2023plant} & - & 78.0 & 2.15  & 16.7  &  77.0 &  1.62 & 12.7  & 76.0 & \textbf{1.06}  & 11.8   
        \\
         & PGD \cite{villegas2024evaluating} & - & 70.17  &  9.8 & 39.1  & 67.6  & 9.83  & 46.9  &  61.2 & 9.7  & 46.2  
        \\
        \midrule
        \multirow{3}{*}{Dgcnn \cite{wang2021object}} & FGSM \cite{sen2023adversarial}  & - & 41.3 & 2.52 & 9.13 & 50.2 & 2.52  & 9.13  & 55.2 & 4.09 & 14.29 
        \\
        & IFGSM \cite{you2023plant} & - & 57.6 & 3.5 & 12.5 &  72.5 & 3.49  & 12.5  & 60.2 & 3.5  & 12.52  
        \\
        & PGD \cite{villegas2024evaluating} & - & 61.6  & 9.63  & 38.1  & 62.5  & 9.73  & 46.9 & 62.8  & 9.8  & 48.3 
        \\
        \midrule
        \multirow{3}{*}{Pct \cite{guo2021pct}} & FGSM \cite{sen2023adversarial} & - &  30 & 3.7  & 14  & 45.2  & 3.75  & 13.9  & 45.6  & 3.2  & 12.4
        \\
        & IFGSM \cite{you2023plant} & - & 44.5  & 5.5  & 19.3  & 72.3  & 5.56  & 19.3 &  64.3 & 5.56  & 19.3
        \\
        & PGD \cite{villegas2024evaluating}& - & 69  & 9.9  & 48.3  &  63.4 & 9.9  & 48  & 63.0  & 9.8  & 48.3        \\
        \midrule
        3D-Diffusion& (DifA) Ours & - & \textbf{86.0}  & \textbf{1.7}  & \textbf{7.4}  & \textbf{87}  &  1.7 & 7.4  & \textbf{86}  & 1.7  & \textbf{7.4} 
        \\
        \bottomrule
    \end{tabular}
    }
    % \vspace{0.5em}
    \label{tab:table1}
    % \vspace{-0.5em}
\end{table*}

\subsection{Results on Defense Approaches}
To further validate the robustness of each attack method, we perform performance evaluation tests on the produced adversarial examples after the defense methods. We consider common point cloud input preprocessing defense methods \cite{tang2023deep}. We demonstrate the superiority of our proposed scheme by testing it against other attack methods (FGSM, IFGSM, PGD). Input defense methods We choose two common input preprocessing schemes (SOR, SRS) for point clouds, The results are shown in Tables \ref{tab:table2} and \ref{tab:table3}. Moreover, the attack effect of our proposed method after SOR defense is almost the highest success rate among all attacks, and it also performs best in Chamfer Distance and Hausdorff Distance. 

\noindent \textbf{Performance comparison under SOR defense approach}
We use the SOR defense method with $k$ set to 2 and $\alpha$ using 1.1 as the defense parameter, and the results obtained show that our proposed scheme still has good aggressiveness after the point cloud defense treatment. In our experiments, we found that if the proxy model is Pointnet, the success rate in attacking PointNet++, Curvenet, and PointConv models is higher than if the proxy model is the other two. Using Dgcnn as the proxy model, the attack performance for Curvenet, PointConv is higher than that for PointNet++. This is an interesting phenomenon, suggesting that point cloud attacks can be ideally achieved by using similar models to generate adversarial examples for robustness tests. And the experimental results show that the attack method based on the diffusion generation model we proposed can produce better attack performance on different models through one-time proxy model generation, and the Chamfer Distance and Hausdorff Distance are smaller than other attack methods, indicating the superiority of our method. \textcolor{blue}{As shown in the figure, we show the visualization of adversarial point clouds of our proposed method and Shape-Invariant(SI) for comparison in Tab \ref{tab:vision-compare}. The SI method is set to $\epsilon$ $=$ 0.16 and step size $=$ 0.007, The noise scale of our method is set to $0.05t$. Our adversarial generation scheme based on the diffusion model has fewer outliers and a smoother surface than the SI attack. Regardless of whether it has been through the point cloud defense method or not, the point cloud quality generated by our adversarial sample generation scheme is better than that of the SI attack.}\jz{has fewer outliers? show statistics. Regardless of through the point cloud or not, it is not good wording. show through the point cloud compared with SI attack, what is the improvement and not through point cloud, what is the improvement}

% \begin{table}[t]
% \centering
% \scalebox{1.1}{
% \begin{tabular}{lll}
% \hspace{0.5cm}\textbf{Clean} & \hspace{0.7cm}\textbf{SI} & \hspace{0.5cm}\textbf{Ours} \vspace{0.02cm}\\
% {\includegraphics[width=1.8cm]{image/sota compari/table.png}} & 
% {\includegraphics[width=1.8cm]{image/sota compari/SIatt.png}} &
% {\includegraphics[width=1.8cm]{image/sota compari/oursdiff.png}} \\
% {\includegraphics[width=1.9cm]{image/sota compari/chair.png}} & 
% {\includegraphics[width=1.9cm]{image/sota compari/SIsordefense-chair.png}} & 
% {\includegraphics[width=1.9cm]{image/sota compari/chair1.png}} \\
% \end{tabular}}
% \caption{Experimental results comparison chart of our proposed solution and SI. Each column refers to a method. \textit{Upper row}: Illustration of an unprotected AEs \textit{Lower row}: Illustration of AEs defended by SOR.
% \label{tab:vision-compare}
% \end{table}

\begin{table}[t]
\centering
\scalebox{1.1}{
\begin{tabular}{lll}
\hspace{0.5cm}\textbf{Clean} & \hspace{0.7cm}\textbf{SI} & \hspace{0.5cm}\textbf{Ours} \\[0.02cm]
\includegraphics[width=1.8cm]{image/sota compari/table.png} & 
\includegraphics[width=1.8cm]{image/sota compari/SIatt.png} &
\includegraphics[width=1.8cm]{image/sota compari/oursdiff.png} \\
\includegraphics[width=1.9cm]{image/sota compari/chair.png} & 
\includegraphics[width=1.9cm]{image/sota compari/SIsordefense-chair.png} & 
\includegraphics[width=1.9cm]{image/sota compari/chair1.png} \\
\end{tabular}}
\caption{Experimental results comparison chart of our proposed solution and SI. Each column refers to a method. \textit{Upper row}: Illustration of an unprotected AEs. \textit{Lower row}: Illustration of AEs defended by SOR.}
\label{tab:vision-compare}
\end{table}




\begin{table*}[!htb]
    % \setlength{\belowcaptionskip}{1cm}
    % \scriptsize
	\footnotesize
    \centering
        \caption{Quantitative comparison between our diff attack and existing black-box transfer-based attacks in terms of attack success rate (ASR), Chamfer distance (CD), Hausdorff distance (HD), the proxy model and defense method SOR used, where CD is multiplied by $10^2$ and HD is multiplied by $10^2$ for better comparison.}
    \setlength{\tabcolsep}{1mm}{
    \begin{tabular}{lcp{10mm}<{\centering}p{10mm}<{\centering}p{10mm}<{\centering}p{10mm}<{\centering}p{10mm}<{\centering}p{10mm}<{\centering}p{10mm}<{\centering}p{10mm}<{\centering}p{10mm}<{\centering}p{10mm}<{\centering}p{10mm}<{\centering}p{10mm}<{\centering}p{10mm}<{\centering}}
        \toprule
        \multirow{3}{*}{Proxy Model}
        & \multirow{3}{*}{Attack}
        & \multirow{3}{*}{Defense}
        & \multicolumn{3}{c}{PointNet++ \cite{qi2017pointnet++}} 
        & \multicolumn{3}{c}{Curvenet \cite{muzahid2020curvenet}}
        & \multicolumn{3}{c}{PointConv \cite{wu2019pointconv}}
        \\
        \cmidrule(lr){4-6}\cmidrule(lr){7-9}\cmidrule(lr){10-12}
        & & & ASR$\uparrow$ & CD$\downarrow$ & HD$\downarrow$ & ASR$\uparrow$ & CD$\downarrow$ & HD$\downarrow$ & ASR$\uparrow$ & CD$\downarrow$ & HD$\downarrow$  
        \\
        & & & (\%) & ($10^{-2}$) & ($10^{-2}$) & (\%) & ($10^{-2}$) & ($10^{-2}$) & (\%) & ($10^{-2}$) & ($10^{-2}$) 
        \\
        \midrule
        \multirow{3}{*}{PointNet} & FGSM \cite{sen2023adversarial}  & \multirow{3}{*}{SOR} &  54.3 & \textbf{1.2}  & 16.3  & 66.5  & 1.6  & \textbf{2.05}  & 54.3  & 1.2  & 16.3  
        \\
        & IFGSM \cite{you2023plant} &  & 75.3  & 4.8  & 38.5  & 80  & 4.3  & 30.5  &  72 & \textbf{1.02}  & 12.2 
        \\
         & PGD \cite{villegas2024evaluating} &  & 69.5  & 9.9  & 48.2   & 82  & 9.95  & 48.2  & 80 & 9.7  & 46.4  
        \\
        \midrule
        \multirow{3}{*}{Dgcnn} & FGSM \cite{sen2023adversarial}  & \multirow{3}{*}{SOR} & 45.05 & 2.72  & 11.68  & 61  & 2.7  & 11.6  &  64.8 & 3.84  & 14.5  
        \\
        & IFGSM \cite{you2023plant} &  &  48.5 & 5.07 & 18.4  & 73.2  & 3.84 & 14.5  &  73 & 3.84   & 14.4   
        \\
        & PGD \cite{villegas2024evaluating} &  & 69.5  & 9.9  & 48.2  & 83  & 9.75  & 48.1  & 82  & 9.8  & 47.6 
        \\
        \midrule
        \multirow{3}{*}{Pct} & FGSM \cite{sen2023adversarial} & \multirow{3}{*}{SOR} & 46.8  & 2.75  & 11.68  & 61.8  & 2.7  &11.6   & 54.9  & 2.7  & 11.6
        \\
        & IFGSM \cite{you2023plant} &   & 47.8  & 5.09  & 18.5  &  77.8 & 5.09  & 18.5  & 65.6  & 5.06  & 18.4
        \\
        & PGD \cite{villegas2024evaluating}&   & 72.7  & 9.8  & 48.3  & 72.5  & 9.8  & 48.3  &  81 & 9.8  & 48.3
        \\
        \midrule
        3D-Diffusion& (DifA)Ours & SOR & \textbf{84.7}  & 1.4  & \textbf{6.8}  & \textbf{86.2}  & \textbf{1.4}  & 6.8  & \textbf{85.0}  & 1.4  & \textbf{6.8} 
        \\
        \bottomrule
    \end{tabular}
    }
    % \vspace{0.5em}
    \label{tab:table2}
    % \vspace{-0.5em}
\end{table*}


==> Body/Method.tex <==


We aim to generate adversarial point clouds by adding perturbations extracted from the latent space of a 3D-diffusion model, then leverage the transferability of generated AEs to fool target model $F_{\theta}$. To enhance the imperceptibility of generated AEs, we constrain the perturbations with Mean Square Error (MSE) and Density-based Chamfer Distance (DCD) \cite{wu2021density} simultaneously. We present the details of AE generation below. The overview of the framework is shown in Fig \ref{fig:overview}.\jz{I think we need to start with an attack model as it is an attack paper. Also I suggest to walk through the main figure here in high-level, for instance, highlight in the figure what are the novelty part of our design, making them I, II, III and then delve-deeper into each of them, explain the novelty in each of these components comparing with the SOTA}
% Starting with a clean point cloud, we identify adversarial distributions from the latent space of the diffusion model, which are then transformed into adversarial noise and added to the clean point cloud. 

% Due to the generative nature of the model, which can produce diverse outputs, we apply constraints to ensure that the added noise remains effective and imperceptible: specifically, we use DCD loss to maintain the geometrical proximity between the transformed and original point clouds, and employ an MSE loss to ensure that the final distribution of the adversarial point cloud does not deviate significantly from the original, thus ensuring that the generated adversarial point clouds are both effective in fooling 3D models and maintain a high degree of similarity to the original point clouds, enhancing their stealthiness and transferability across different models.

\begin{figure*}[!t]
    \centering
    \includegraphics[width=1\textwidth]{image/3d.drawio (2).pdf}
    \caption{Basic framework structure}
    \label{fig:overview}
\end{figure*}



\subsection{Problem Formulation}
Given a clean point cloud $X$ and a well-trained target model $F_{\theta}$ for point cloud recognition, an adversary aims to fool the model $F_{\theta}$ by adding negligible perturbations $\delta$ to the clean sample: $F_{\theta}(X+\delta) \neq y$, where $\theta$ refers to the model parameters and $y$ is the correct label. 

\subsection{Latent Representation $z$}
Our goal is to add adversarial noise to the clean point cloud through the diffusion model. We first need carefully trained prior knowledge $z$ to guide the diffusion model to add noise points to achieve this goal. This prior distribution can be derived from other real point cloud classifications. Specifically, we first use VAE to train a self-supervised model to obtain the latent representation of other classified point clouds, i.e. z. The detailed VAE is shown in \cite{diffusion3D}. The latent representation can be considered as the compressed features of other classified point clouds. Then we use $z$ to supervise the reverse noise addition process of the diffusion model to produce adversarial samples.
\subsection{Reverse Diffusion For Point Clouds}
After training and obtaining the VAE’s latent representation, we use reverse diffusion to add noise to the point cloud. For the adversarial addition process of the clean point cloud, We introduce the reverse diffusion process into adversarial point cloud generation to produce transferable adversarial samples. At each step of the reverse diffusion process, appropriate noise is added based on the current point cloud features, generating point clouds highly similar to the original distribution $z$. By iteratively applying this process, the diffusion model can generate realistic samples. Utilizing this property, we use clean point clouds as the input for reverse diffusion and guide the process using data distribution \( z \) that does not belong to the current point cloud classification. This \( z \) is obtained as a prior distribution through training a self-supervised model with VAE, supervising the reverse diffusion process. This ensures that each step of diffusion, represented as \( p(x_i^T) \), includes adversarial points sampled from distributions other than the approximate input points. This method allows us to add noise to clean point clouds, transforming the reverse diffusion process into an adversarial noise addition process.
\begin{multline}
p_{\boldsymbol{\theta}}\left(\boldsymbol{x}^{(0: T)} \mid \boldsymbol{z}\right) = p\left(\boldsymbol{x}^{(T)}\right) \prod_{t = 1}^{T} p_{\boldsymbol{\theta}}\left(\boldsymbol{x}^{(t-1)} \mid \boldsymbol{x}^{(t)}, \boldsymbol{z}\right), \\
p_{\boldsymbol{\theta}}\left(\boldsymbol{x}^{(t-1)} \mid \boldsymbol{x}^{(t)}, \boldsymbol{z}\right) = \mathcal{N}\left(\boldsymbol{x}^{(t-1)} \mid \boldsymbol{\mu}_{\boldsymbol{\theta}}\left(\boldsymbol{x}^{(t)}, t, \boldsymbol{z}\right), \beta_{t} \boldsymbol{I}\right),\,
\end{multline}
where $\mu_\theta$ is the estimated mean implemented by a neural network parameterized by $\theta$. $z$ is the shape latent control the noise. The starting $p(x_i^{T})$ is set to a clean input. We obtain the adversarial examples with the latent shape $z$ by passing a set of points sampled from $p(x_i^{T})$ through the reverse process.
\subsection{Suppressing The Diversity Of Diffusion Model}
To prevent the initial point cloud from losing its original shape due to the strong recovery capability of the reverse diffusion process and to avoid the generation of excessive outlier points, we employ a DCD (Density-aware Chamfer Distance) optimization that increases with each reverse diffusion step. This optimization controls the diffusion process to ensure consistency between each successive point cloud. By doing so, the structural integrity of the point cloud is excellently preserved throughout the diffusion process, facilitating the generation of adversarial point clouds that are both covert and effective. We demonstrate the effect of this in the subsequent experiment result section. The Density-aware Chamfer Distance (DCD) is defined as follows:
\begin{multline}
l_{DCD}\left(X, X^{'}\right)=\frac{1}{2}\left(\frac{1}{\left|X\right|} \sum_{x \in X}\left(1-\frac{1}{n_{\hat{y}}} e^{-\alpha|| x-\hat{y} \|_{2}}\right)\right.
\\ \left.+\frac{1}{\left|X^{'}\right|} \sum_{y \in X^{'}}\left(1-\frac{1}{n_{\hat{x}}} e^{-\alpha|| y-\hat{x} \|_{2}}\right)\right),
\end{multline}
as it can detect the difference in density distribution and takes into account the overall structure and local geometric details of the point cloud, we use this distance to control the variability between the adversarial point cloud and the original point cloud, acting on the diffusion process, where $\hat{y} = min_{y \in X^{'}}|| x-y \|_{2}$, $\hat{x} = min_{y \in X}|| y-x \|_{2}$, and $\alpha$ denotes a temperature scalar. Here $n_{\hat{y}} = |X_1^y|$, Each $y$ contributes $\left|-\frac{1}{n_{y}} \sum_{x \in X^{y}} e^{-\|x-y\|_{2}}\right| \in[0,1]$ to the overall distance metric before averaging. This integration ensures that the generated adversarial samples remain imperceptible while effectively deceiving the classification model, thus enhancing the robustness and effectiveness of the diffusion attack scheme.

\begin{figure*}[!t]
    \centering
    \includegraphics[scale=0.5, keepaspectratio]{image/experiment_result.jpg}
    \caption{Point cloud data visualization comparison (clean vs. attacked point cloud)}
    \label{fig:experiment_result}
\end{figure*}


To further improve the smoothness of the generated point cloud, we use the Mean Squared Error (MSE) loss function to remove outliers and balance error treatment. MSE's simplicity aids in stable gradient descent and effective convergence, but it treats all points equally and may miss finer structural details. During the diffusion process, we use DCD instead of MSE because DCD maintains spatial coherence and reduces excessive outliers by focusing on the local structure of the point cloud. For final optimization, MSE is used to ensure global alignment. This balanced approach leverages DCD for local integrity during diffusion and MSE for overall alignment, resulting in high-quality adversarial point clouds with preserved geometric features. We present the results with different loss settings in subsequent ablation experiments. The MSE is defined as follows:
\begin{equation}
    \operatorname{l_{MSE}}\left(X, X^{\prime}\right)=\frac{1}{n} \sum_{i=1}^{n}\left\|X_{i}-X_{i}^{\prime}\right\|_{2}^{2}.
\end{equation}
Here, \(X\) represents the original point cloud, while \(X'\) denotes the generated adversarial point cloud. The \(n\) stands for the total number of points in the point cloud, and \(X_i\) and \(X'_i\) are the \(i\)-th points in the original and generated point clouds, respectively. The \(\| \cdot \|_2\) is the Euclidean norm, measuring the distance between corresponding points. The term \(\| X_i - X'_i \|_2^2\) represents the squared Euclidean distance between \(X_i\) and \(X'_i\), quantifying the error for each point pair. The expression \(\frac{1}{n} \sum_{i=1}^{n}\) averages the total error across all point pairs, providing a comprehensive measure of alignment quality. Minimizing MSE ensures that the generated adversarial point cloud closely aligns with the original, maintaining structural integrity while effectively evaluating and enhancing attack and defense strategies. 

==> Body/Preliminary.tex <==
We focus on AE generation in the context of point cloud classification tasks. We denote $D=\{X_{i},y_i\}_{i=1}^n$ as the dataset of point clouds. We use $X_i\in R^{m\times3}$ to represent a single point cloud to be classfied in $D$, which contains a set of unordered point sets, and $y_i$ is the corresponding label. The goal of this work is to introduce a small perturbation $\delta_i$ to the point cloud $X_i$, causing the classifier $F_\theta$ to have incorrect classification results for point cloud $X_i$. The formula is as follows:
\begin{equation}
    F_{\theta_i}(X+\delta_i) \neq y_i.
\end{equation}

\begin{equation}
    \delta=X^{T}-reverse(X^T \to X^{T-1}).
\end{equation}



In order to obtain more imperceptible adversarial point 
clouds $X^{'}=X+\delta$, our attack process adopts optimization algorithm, which can be formulated as:

\begin{equation}
    \min \lambda * \mathcal{L}_{DIS}(X,X^{'}),
\end{equation}

where $\mathcal{L}_{dis}$ is a regularization
term constraining the distance between benign point cloud
$X$ and the adversarial one $X^{'}$

\textbf{Problem Analysis. }The adversarial perturbation is added by the back-diffusion process of the diffusion model. Since each back-diffusion generation of the diffusion model can generate samples similar to the previous step, based on this feature, we assume that the back-diffusion process can generate an adversarial point cloud that is close to the sample point cloud of the previous step. After iterating this process, we generate the adversarial examples we need. In order to limit the added perturbation $\delta$ from being too large, resulting in unexpected deformation of the generated adversarial samples, we use $\mathcal{L}_{DCD}$ and $\mathcal{L}_{MSE}$ to control the size of the perturbation. At the same time, this approach can prevent the original shape of the point cloud from being destroyed due to the generation diversity of the generation model itself. Based on this idea, we propose an adversarial sample generation scheme based on the diffusion model, and the specific approach will be explained in detail in the next section.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~(\ref{#1})}
% Reference to an equation, upper case
\def\Eqref#1{Equation~(\ref{#1})}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}
\def\vdelta{{\bm{\delta}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak
